Fast Ensembling with Diffusion Schr\"odinger Bridge

Deep Ensemble (DE) approach is a straightforward technique used to enhance the performance of deep neural networks by training them from different initial points, converging towards various local optima. However, a limitation of this methodology lies in its high computational overhead for inference, arising from the necessity to store numerous learned parameters and execute individual forward passes for each parameter during the inference stage. We propose a novel approach called Diffusion Bridge Network (DBN) to address this challenge. Based on the theory of the Schr\"odinger bridge, this method directly learns to simulate an Stochastic Differential Equation (SDE) that connects the output distribution of a single ensemble member to the output distribution of the ensembled model, allowing us to obtain ensemble prediction without having to invoke forward pass through all the ensemble models. By substituting the heavy ensembles with this lightweight neural network constructing DBN, we achieved inference with reduced computational cost while maintaining accuracy and uncertainty scores on benchmark datasets such as CIFAR-10, CIFAR-100, and TinyImageNet. Our implementation is available at https://github.com/kim-hyunsu/dbn.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/c10.tex <==
\begin{table*}[h]
    \newcommand{\metricrule}{\cmidrule(lr){2-3} \cmidrule(lr){4-8}}
    \newcommand{\modelrule}{\cmidrule(lr){1-8}}
    \renewcommand{\arraystretch}{1.18}
    \centering
    \caption{
        Performance on CIFAR-10 dataset.
    }
    \vspace{-2mm}
    \resizebox{\textwidth}{!}{
        \begin{tabular}{lrrllllll}
            \\
            \textbf{CIFAR-10} \\
            \toprule
            Model                 & \dmet{FLOPs} & \dmet{\#Params} & \umet{ACC}          & \dmet{NLL}           & \dmet{BS}           & \dmet{ECE}            & \umet{DEE}           \\
            
            \midrule
            
            ResNet (\gls{de}-1)   & \relv{1.000} & \relv{1.000}    & \tv[n]{91.30}{00.10} & \tv[n]{0.3382}{0.0023} & \tv[n]{0.1409}{0.0011} & \tv[n]{0.0658}{0.0003} & \tv[n]{1.000}{}      \\

            \metricrule

            \quad +2 \gls{bn}\textsubscript{small} (\gls{de}-3)  & \relv{1.125} & \relv{1.097}    & \tv[n]{91.79}{00.05} & \tv[n]{0.2579}{0.0009} & \tv[n]{0.1198}{0.0003} & \tv[n]{0.0599}{0.0037} & \tv[n]{1.899}{}      \\

            \quad +4 \gls{bn}\textsubscript{small} (\gls{de}-5)  & \relv{1.245} & \relv{1.283}    & \tv[n]{91.87}{00.05} & \tv[n]{0.2580}{0.0010} & \tv[n]{0.1195}{0.0004} & \tv[n]{0.0624}{0.0098} & \tv[n]{1.898}{}      \\

            \quad +2 \gls{bn}\textsubscript{medium} (\gls{de}-3)  & \relv{1.411} & \relv{1.319}    & \tv[n]{91.91}{00.04} & \tv[n]{0.2544}{0.0011} & \tv[n]{0.1182}{0.0005} & \tv[b]{0.0591}{0.0096} & \tv[n]{1.938}{}      \\
            
            \quad +1 \gls{dbn} (\gls{de}-3)  & \relv{1.166} & \relv{1.213}    & \tv[b]{92.98}{00.16} & \tv[b]{0.2403}{0.0027} & \tv[b]{0.1084}{0.0013} & \tv[n]{0.0666}{0.0010} & \tv[b]{2.363}{}      \\

            \quad +2 \gls{dbn} (\gls{de}-5) & \relv{1.332} & \relv{1.426}    & \tv[b]{93.23}{00.07} & \tv[b]{0.2247}{0.0005} & \tv[b]{0.1033}{0.0005} & \tv[n]{0.0662}{0.0009} & \tv[b]{3.031}{}      \\

            \gls{ed} (\gls{de}-3)            & \relv{1.000} & \relv{1.000}    & \tv[n]{91.96}{00.42} & \tv[n]{0.3505}{0.0214} & \tv[n]{0.1366}{0.0074} & \tv[n]{0.0674}{0.0037} & \tv[n]{$<$1}{}      \\

            \gls{ed} (\gls{de}-5)            & \relv{1.000} & \relv{1.000}    & \tv[n]{91.86}{00.21} & \tv[n]{0.3577}{0.0083} & \tv[n]{0.1391}{0.0031} & \tv[n]{0.0683}{0.0017} & \tv[n]{$<$1}{}      \\

            \gls{end2} (\gls{de}-3)        & \relv{1.000} & \relv{1.000}    & \tv[n]{91.99}{00.14} & \tv[n]{0.3405}{0.0079} & \tv[n]{0.1358}{0.0026} & \tv[n]{0.0690}{0.0013} & \tv[n]{$<$1}{}      \\
            
            \gls{end2} (\gls{de}-5)        & \relv{1.000} & \relv{1.000}    & \tv[n]{92.11}{00.23} & \tv[n]{0.3313}{0.0057} & \tv[n]{0.1336}{0.0029} & \tv[n]{0.0645}{0.0014} & \tv[n]{1.077}{}      \\

            \gls{de}-2            & \relv{2.000} & \relv{2.000}    & \tv[n]{92.72}{00.13} & \tv[n]{0.2489}{0.0031} & \tv[n]{0.1125}{0.0012} & \tv[b]{0.0484}{0.0010} & \tv[n]{2.000}{}      \\
            
            \gls{de}-3            & \relv{3.000} & \relv{3.000}    & \tv[b]{93.06}{00.14} & \tv[b]{0.2252}{0.0024} & \tv[b]{0.1038}{0.0008} & \tv[b]{0.0469}{0.0012} & \tv[b]{3.000}{}      \\

            \gls{de}-5            & \relv{5.000} & \relv{5.000}    & \tv[b]{93.61}{00.11} & \tv[b]{0.2005}{0.0015} & \tv[b]{0.0951}{0.0004} & \tv[b]{0.0466}{0.0009} & \tv[b]{5.000}{}      \\
            \bottomrule
        \end{tabular}
    }
    \label{tab:c10}
\end{table*}


==> tables/c100.tex <==
\begin{table*}[t]
    \newcommand{\metricrule}{\cmidrule(lr){2-3} \cmidrule(lr){4-8}}
    \newcommand{\modelrule}{\cmidrule(lr){1-8}}
    \renewcommand{\arraystretch}{1.18}
    \centering
    \caption{
        Performance on CIFAR-100 dataset.
    }
    \vspace{-2mm}
    \resizebox{\textwidth}{!}{
        \begin{tabular}{lrrllllll}
            \\
            \toprule
            Model                 & \dmet{FLOPs} & \dmet{\#Params} & \umet{ACC}          & \dmet{NLL}           & \dmet{BS}           & \dmet{ECE}            & \umet{DEE}           \\
            
            \midrule

            ResNet (\gls{de}-1)   & \relv{1.000} & \relv{1.000}    & \tv[n]{72.29}{00.36} & \tv[n]{1.1506}{0.0100} & \tv[n]{0.4001}{0.0044} & \tv[n]{0.1526}{0.0005} & \tv[n]{1.000}{}      \\
            
            \metricrule

            \quad +2 \gls{bn}\textsubscript{medium} (\gls{de}-3)  & \relv{1.419} & \relv{1.320}    & \tv[n]{74.97}{00.05} & \tv[n]{1.0360}{0.0022} & \tv[n]{0.3500}{0.0007} & \tv[n]{}{} & \tv[n]{1.642}{}      \\

            \quad +1 \gls{dbn} (\gls{de}-3)  & \relv{1.166} & \relv{1.213}    & \tv[b]{76.02}{00.11} & \tv[b]{0.9434}{0.0051} & \tv[b]{0.3438}{0.0009} & \tv[b]{0.1352}{0.0020} & \tv[b]{2.461}{}      \\

            \quad +2 \gls{dbn} (\gls{de}-5) & \relv{1.332} & \relv{1.426}    & \tv[b]{76.82}{00.22} & \tv[b]{0.8998}{0.0046} & \tv[b]{0.3305}{0.0018} & \tv[b]{0.1269}{0.0013} & \tv[b]{3.297}{}      \\

            \gls{ed} (\gls{de}-3)            & \relv{1.000} & \relv{1.000}    & \tv[n]{74.18}{00.22} & \tv[n]{1.2375}{0.0125} & \tv[n]{0.4095}{0.0019} & \tv[n]{0.1819}{0.0013} & \tv[n]{$<$1}{}      \\

            \gls{ed} (\gls{de}-5)            & \relv{1.000} & \relv{1.000}    & \tv[n]{74.00}{00.29} & \tv[n]{1.2428}{0.0174} & \tv[n]{0.4120}{0.0041} & \tv[n]{0.1840}{0.0022} & \tv[n]{$<$1}{}      \\

            \gls{end2} (\gls{de}-3)        & \relv{1.000} & \relv{1.000}    & \tv[n]{73.35}{00.22} & \tv[n]{1.3572}{0.0079} & \tv[n]{0.4350}{0.0013} & \tv[n]{0.1973}{0.0006} & \tv[n]{$<$1}{}      \\
            
            \gls{end2} (\gls{de}-5)        & \relv{1.000} & \relv{1.000}    & \tv[n]{73.22}{00.33} & \tv[n]{1.3597}{0.0156} & \tv[n]{0.4370}{0.0052} & \tv[n]{0.1980}{0.0030} & \tv[n]{$<$1}{}      \\

            \gls{de}-2            & \relv{2.000} & \relv{2.000}    & \tv[n]{74.98}{00.42} & \tv[n]{0.9721}{0.0099} & \tv[n]{0.3505}{0.0034} & \tv[n]{0.1259}{0.0021} & \tv[n]{2.000}{}      \\
            
            \gls{de}-3            & \relv{3.000} & \relv{3.000}    & \tv[b]{76.04}{00.13} & \tv[b]{0.9098}{0.0019} & \tv[b]{0.3342}{0.0007} & \tv[b]{0.1233}{0.0020} & \tv[b]{3.000}{}      \\

            \gls{de}-5            & \relv{5.000} & \relv{5.000}    & \tv[b]{77.03}{00.08} & \tv[b]{0.8606}{0.0036} & \tv[b]{0.3216}{0.0013} & \tv[b]{0.1234}{0.0019} & \tv[b]{5.000}{}      \\
            
            \bottomrule
        \end{tabular}
    }
    \label{tab:c100}
\end{table*}


==> tables/t200.tex <==
\begin{table*}[t]
    \newcommand{\metricrule}{\cmidrule(lr){2-3} \cmidrule(lr){4-8}}
    \newcommand{\modelrule}{\cmidrule(lr){1-8}}
    \renewcommand{\arraystretch}{1.18}
    \centering
    \caption{
        Performance on TinyImageNet dataset.
    }
    \vspace{-2mm}
    \resizebox{\textwidth}{!}{
        \begin{tabular}{lrrllllll}
            \\
            \toprule
            Model                 & \dmet{FLOPs} & \dmet{\#Params} & \umet{ACC}          & \dmet{NLL}           & \dmet{BS}           & \dmet{ECE}            & \umet{DEE}           \\
            
            \midrule
            
            ResNet (\gls{de}-1)   & \relv{1.000} & \relv{1.000}    & \tv[n]{59.26}{00.23} & \tv[n]{1.8399}{0.0294} & \tv[n]{0.5438}{0.0076} & \tv[n]{0.1671}{0.0091} & \tv[n]{1.000}{}      \\
            
            \metricrule

            \quad +2 \gls{bn}\textsubscript{medium} (\gls{de}-3)  & \relv{1.359} & \relv{1.412}    & \tv[n]{00.00}{00.00} & \tv[n]{0.0000}{0.0000} & \tv[n]{0.0000}{0.0000} & \tv[n]{}{} & \tv[n]{0.000}{}      \\

            \quad +1 \gls{dbn} (\gls{de}-3)  & \relv{1.209} & \relv{1.149}    & \tv[b]{64.25}{00.35} & \tv[b]{1.5542}{0.0045} & \tv[b]{0.4768}{0.0024} & \tv[b]{0.1862}{0.0017} & \tv[b]{2.893}{}      \\

            \quad +2 \gls{dbn} (\gls{de}-5) & \relv{1.418} & \relv{1.398}    & \tv[b]{64.73}{00.10} & \tv[b]{1.5247}{0.0045} & \tv[b]{0.4702}{0.0016} & \tv[b]{0.1838}{0.0019} & \tv[b]{3.586}{}      \\

            \gls{ed} (\gls{de}-3)            & \relv{1.000} & \relv{1.000}    & \tv[n]{60.81}{00.26} & \tv[n]{1.8312}{0.0129} & \tv[n]{0.5443}{0.0052} & \tv[n]{0.2126}{0.0021} & \tv[n]{$<$1}{}      \\

            \gls{end2} (\gls{de}-3)        & \relv{1.000} & \relv{1.000}    & \tv[n]{60.81}{00.26} & \tv[n]{1.3572}{0.0079} & \tv[n]{0.4350}{0.0013} & \tv[n]{0.1973}{0.0006} & \tv[n]{$<$1}{}      \\

            \gls{de}-2            & \relv{2.000} & \relv{2.000}    & \tv[n]{62.49}{00.24} & \tv[n]{1.6219}{0.0046} & \tv[n]{0.4929}{0.0015} & \tv[n]{0.1404}{0.0011} & \tv[n]{2.000}{}      \\
            
            \gls{de}-3            & \relv{3.000} & \relv{3.000}    & \tv[b]{64.00}{00.27} & \tv[b]{1.5461}{0.0086} & \tv[b]{0.4769}{0.0026} & \tv[b]{0.1384}{0.0011} & \tv[b]{3.000}{}      \\
            
            \bottomrule
        \end{tabular}
    }
    \label{tab:t200}
\end{table*}

